Learning Preconditioner for Conjugate Gradient PDE Solvers

Efficient numerical solvers for partial differential equations empower science and engineering. One of the commonly employed numerical solvers is the preconditioned conjugate gradient (PCG) algorithm which can solve large systems to a given precision level. One challenge in PCG solvers is the selection of preconditioners, as different problem-dependent systems can benefit from different preconditioners. We present a new method to introduce \emph{inductive bias} in preconditioning conjugate gradient algorithm. Given a system matrix and a set of solution vectors arise from an underlying distribution, we train a graph neural network to obtain an approximate decomposition to the system matrix to be used as a preconditioner in the context of PCG solvers. We conduct extensive experiments to demonstrate the efficacy and generalizability of our proposed approach in solving various 2D and 3D linear second-order PDEs.

==> sections/intro.tex <==
\section{Introduction}\label{sec:intro}

Partial differential equations (PDEs) are fundamental mathematical models with broad applications in science and engineering, for example, the Navier-Stokes equation in fluid dynamics, Poisson's equation in computational geometry, and the Black–Scholes equation in mathematical finance. Despite their powerful modeling ability and wide applications, it is notoriously difficult to find analytical solutions to a general PDE. Therefore, numerical solvers have long been the mainstay of solving PDEs. Classic PDE solvers provide accurate solutions to well-understood PDEs but typically at the cost of long computation time. Speeding up these classic solvers is non-trivial and often requires complex numerical techniques, e.g., multi-grid methods \citep{briggs2000multigrid}, domain decomposition \citep{smith1997domain}, and model reduction \citep{holmes2012turbulence}. Recently, several pioneering works \citep{li2018learning,sanchez2020learning} introduce machine learning techniques to solving PDEs, particularly in the field of physics simulation. While this line of methods typically outperforms classic solvers in speed by a large margin, it struggles with converging into a highly precise solution (e.g., $1e-12$). A lack of theoretical analysis on convergence and accuracy inhibits neural-network PDE solvers' applications in mechanical engineering, structure analysis, and aerodynamics, where precise PDE solutions have a higher priority than fast yet inexact results.

%\td{Paragraph 3: explain our intuition and approach.}
This work proposes NeuralPCG, a novel and hybrid method that combines the benefits of classic and machine-learning PDE solvers. Our key observation is that neural-network solvers are fast at estimating PDE solutions with a low to moderate accuracy. This property aligns with the \emph{preconditioning} technique in numerical methods, which uses an easy-to-solve approximation of the original PDE to speed up numerical solvers. Based on this intuition, NeuralPCG proposes to learn a neural network that \emph{preconditions} a classic iterative solver. This is in sharp contrast to existing neural-network PDE solvers that replace the numerical solver entirely with a neural network. The backbone of NeuralPCG remains to be a classic solver, empowering it to inherit convergence and accuracy guarantees. Moreover, the learned preconditioner even outperforms classic preconditioners because it adapts to data distributions from target PDE applications.

%\td{Paragraph 4: describe the evaluation results.}
To demonstrate the efficacy of NeuralPCG, we evaluate it on a set of 2D and 3D representative linear second-order PDEs. We compare its performance with two baselines of very different natures: (1)the preconditioned conjugate gradient (PCG) algorithm with classic preconditioners; (2) MeshGraphNet (MGN), a state-of-the-art neural-network PDE solver \citep{pfaff2020learning}. Our experiments show that NeuralPCG has its unique advantage over both baselines: Compared with MGN and similar machine-learning solvers, NeuralPCG generates convergent and accurate solutions by construction and avoids error accumulation. On the other hand, NeuralPCG also outperforms classic PCG solvers in speed because it learns a preconditioner tailored to the training data distribution, which classic preconditioners typically do not exploit. Finally, NeuralPCG generalizes to physics parameters or meshes with moderate differences ($5\sigma$) from the training data and is robust to outliers by design.

%\td{Paragraph 5: summarize the contributions.}
In summary, our work makes the following contributions:
\begin{enumerate}
    \item We propose NeuralPCG, a novel and efficient solver for linear second-order PDEs that combines the benefits of classic and machine-learning PDE solvers.
    \item We present a framework for studying the performance of preconditioners in classic iterative solvers, including a benchmark problem set with carefully designed performance metrics.
    \item We conduct extensive experiments to evaluate the efficacy and generalizability of NeuralPCG and demonstrate its advantages over existing methods.
\end{enumerate}

==> table/4-1-synthetic-time.tex <==
% 	\hspace{-5mm}
	\begin{table*}[t]
% 	\footnotesize{
        % \small 
     \resizebox{\textwidth}{!}{%
        \scriptsize
		\begin{center}
			\begin{tabular}{c|ccccc|ccccc|cc}
				\toprule
				& \multicolumn{5}{c}{Heat Equation} & \multicolumn{5}{c}{ Poisson Equation} \\
				\midrule
				% \hline
				% \hline % \midrule 
				& 1e-4 & 1e-6  & 1e-8  & 1e-10  & 1e-12 & 1e-14 & 1e-16 & Area \\
				  \midrule				% \hline
				Identity&  &  &  &  &  &  &  &  &  &  &  &   \\
				% \hline % \midrule				
				Jacobi &  &  &  &  &  &  &  &  &  & &  &  \\
				% \hline %\midrule				
				IC &  &  &  &  &  &  &  &  &  &  &  &   \\
				% \hline %\midrule				
				Ours no pred_x &  &  &  &  &  &  &  &  &  &  &  &     \\
			    
				Ours with pred_x &  &  &  &  &  &  &  &  &  &  &  &     \\
		
				\bottomrule
			\end{tabular}
		\end{center}
	} % resizebox
		\caption{Quantitative comparison number of CG iteration}
		\label{table:performance}
% 		}
% 		\vspace{-0.2cm}
	\end{table*}	

==> table/4-2-simulation-time.tex <==
% 	\hspace{-5mm}
	\begin{table*}[t]
% 	\footnotesize{
        % \small 
     \resizebox{\textwidth}{!}{%
        \scriptsize
		\begin{center}
			\begin{tabular}{c|ccccc|ccccc|cc}
				\toprule
				& \multicolumn{5}{c}{Heat Equation} & \multicolumn{5}{c}{ Poisson Equation} \\
				\midrule
				% \hline
				% \hline % \midrule 
				& 1e-4 & 1e-6  & 1e-8  & 1e-10  & Area  & 1e-4 & 1e-6  & 1e-8  & 1e-10  & Area \\
				  \midrule				% \hline
				Identity&  &  &  &  &  &  &  &  &  &  &  &   \\
				% \hline % \midrule				
				Jacobi &  &  &  &  &  &  &  &  &  & &  &  \\
				% \hline %\midrule				
				IC &  &  &  &  &  &  &  &  &  &  &  &   \\
				% \hline %\midrule				
				Ours &  &  &  &  &  &  &  &  &  &  &  &     \\
			
				\bottomrule
			\end{tabular}
	    
		\end{center}
	} % resizebox
		\caption{Quantitative comparison number of CG iteration}
		\label{table:performance}
% 		}
% 		\vspace{-0.2cm}
	\end{table*}	
	
	
	% 	\hspace{-5mm}
	\begin{table*}[t]
% 	\footnotesize{
        % \small 
     \resizebox{\textwidth}{!}{%
        \scriptsize
		\begin{center}
			\begin{tabular}{c|ccccc|ccccc|cc}
				\toprule
				& \multicolumn{5}{c}{Heat Equation} & \multicolumn{5}{c}{ Poisson Equation} \\
				\midrule
				% \hline
				% \hline % \midrule 
				& 1e-4 & 1e-6  & 1e-8  & 1e-10  & Area  & 1e-4 & 1e-6  & 1e-8  & 1e-10  & Area \\
				  \midrule				% \hline
				Identity& 0.015 & 0.013 & 0.008 & 32.8 & 30.1 & 33.6 & 0.712 & 0.847 & 0.667 & 13.4 & 15.8 & 10.7  \\
				% \hline % \midrule				
				Jacobi & 0.017 & 0.026 & 0.007 & 39.4 & 22.5 & 44.4 & 0.756 & 0.728 & 0.651 & 17.0 & 13.2 & 14.8  \\
				% \hline %\midrule				
				IC & 0.028 & 0.034 & 0.222 & 11.0 & 5.33 & 0.0 & 0.901 & 0.977 & 1.074 & 7.54 & 8.30 & 23.6  \\
				% \hline %\midrule				
				Ours & 0.007 & 0.008 & 0.006 & 65.3 & 61.4 & 45.0 & 0.725 & 0.855 & 0.683 & 24.4 & 30.0 & 18.6    \\
			
				\bottomrule
			\end{tabular}
	    
		\end{center}
	} % resizebox
		\caption{CG Wall Clock Time}
		\label{table:performance}
% 		}
% 		\vspace{-0.2cm}
	\end{table*}	
